Syntactic Completions with Material Obligations

Code editors provide essential services that help developers understand, navigate, and modify programs. However, these services often fail in the presence of syntax errors. Existing syntax error recovery techniques, like panic mode and multi-option repairs, are either too coarse, e.g. in deleting large swathes of code, or lead to a proliferation of possible completions. This paper introduces $\texttt{tall}~\texttt{tylr}$, an error-handling parser and editor generator that completes malformed code with $\textit{syntactic obligations}$ that abstract over many possible completions. These obligations generalize the familiar notion of holes in structure editors to cover missing operands, operators, delimiters, and sort transitions. $\texttt{tall}~\texttt{tylr}$ is backed by a novel theory of tile-based parsing, conceptually organized around a $\textit{molder}$ that turns tokens into tiles and a $\textit{melder}$ that completes and parses tiles into terms using an error-handling generalization of operator-precedence parsing. We formalize melding as a parsing calculus, $\textsf{meldr}$, that completes input tiles with additional obligations such that it can be parsed into a well-formed term, with success guaranteed over all inputs. We further describe how $\texttt{tall}~\texttt{tylr}$ implements molding and completion-ranking using the principle of $\textit{minimizing obligations}$. Obligations offer a useful way to scaffold internal program representations, but in $\texttt{tall}~\texttt{tylr}$ we go further to investigate the potential of $\textit{materializing}$ these obligations visually to the programmer. We conduct a user study to evaluate the extent to which an editor like $\texttt{tall}~\texttt{tylr}$ that materializes syntactic obligations might be usable and useful, finding both points of positivity and interesting new avenues for future work.

==> fig/camel-syntax.tex <==
\begin{figure}
  \newcommand{\ggtrdot}{\textcolor{gray}{\gtrdot}}
  \newcommand{\gvert}{\textcolor{gray}{\vert}}
  \newcommand{\glp}{\textcolor{gray}{(}}
  \newcommand{\glr}{\textcolor{gray}{)}}
  \newcommand{\gplus}[1]{\glp#1\textcolor{gray}{\glr^+}}
  \newcommand{\gstr}[1]{\glp#1\textcolor{gray}{\glr^*}}
  \newcommand{\gopt}[1]{\glp#1\textcolor{gray}{\glr ?}}
  \centering
  \begin{minipage}[t]{0.45\textwidth}
  \[\arraycolsep=3pt\begin{array}{rccl}
    \text{\sortname{expression}} & e & \textcolor{gray}{::=} & n ~\gvert~ x ~\gvert~ \texttt{(}e\texttt{)} ~\gvert~ \texttt{[}\gopt{e\gstr{\texttt{;}~ e}}\texttt{]} \\
    & & \ggtrdot & e\texttt{(}e\texttt{)} \\
    & & \ggtrdot & \texttt{-}e \\
    & & \ggtrdot & e~\texttt{*}~e ~\gvert~ e~\texttt{/}~e \\
    & & \ggtrdot & e~\texttt{+}~e ~\gvert~ e~\texttt{-}~e \\
    % & & \ggtrdot & e~\texttt{|>}~e \\
    & & \ggtrdot & e\gplus{\texttt{,}~ e} \\
    & & \ggtrdot & \texttt{fun}~p~\texttt{=>}~e \\
    & & \gvert & \texttt{let}~p~\texttt{=}~e~\texttt{in}~e\\
    & & \gvert & \texttt{if}~e~\texttt{then}~e~\texttt{else}~e\\
  \end{array}\]
  \end{minipage}
  \begin{minipage}[t]{0.45\textwidth}
    \[\arraycolsep=3pt\begin{array}{rccl}
    \text{\sortname{pattern}} & p & \textcolor{gray}{::=} & n ~\gvert~ x ~\gvert~ \texttt{(}p\texttt{)}
 \\
 & & \ggtrdot & p\texttt{: }\tau \\
 & & \ggtrdot & p\gplus{\texttt{,}}~ p
 \\
 & & \\
    \text{\sortname{type}} & \tau & \textcolor{gray}{::=} & \texttt{Int} ~\gvert~ \texttt{(}\tau\texttt{)}\\
    & & \ggtrdot & \tau \texttt{ -> } \tau
  \end{array}\]
    \end{minipage}
  \caption{A fragment of the concrete syntax of Hazel, an expression-oriented language used for running examples. Here, $n$ ranges over integer literals and $x$ over variable identifiers, specified in the usual way.
  The operator $\ggtrdot$ indicates forms to its left have greater precedence than those to its right. We omit associativity specifications.}
  \label{fig:camel-syntax}
\end{figure}

% \newcommand{\gr}[1]{\textcolor{gray}{#1}}
% \begin{figure}
%   \[\arraycolsep=10pt\begin{array}{rcl}
%     & n & \\
%     \gr{e} * \gr{e},~ \gr{e}\gr{(e}) & * & \langle\rangle,~ (\gr{\langle\rangle)},~ \gr{\langle\rangle}(\gr{e)},~ \texttt{fun}~\gr{p~\texttt{->}~e} \\
%     & ( & \gr{e}~\rangle\langle~\gr{e} \\
%     & root & \gr{e}~\rangle\langle~\gr{e}
%   \end{array}\]
% \caption{neq table}
% \end{figure}

==> fig/grammars.tex <==
\newcommand{\ggtrdot}{\textcolor{gray}{\gtrdot}}
\newcommand{\gvert}{\textcolor{gray}{\vert}}
\newcommand{\glp}{\textcolor{gray}{(}}
\newcommand{\glr}{\textcolor{gray}{)}}
\newcommand{\gplus}[1]{\glp#1\textcolor{gray}{\glr^+}}
\newcommand{\gstr}[1]{\glp#1\textcolor{gray}{\glr^*}}
\newcommand{\gopt}[1]{\glp#1\textcolor{gray}{\glr ?}}
\newcommand{\g}[1]{\textcolor{gray}{#1}}

\newcommand{\gbl}{\textcolor{gray}{\{}}
\newcommand{\gbr}{\textcolor{gray}{\}}}
\newcommand{\gsc}{\textcolor{gray}{;}}

\begin{figure}
  \centering
  \begin{minipage}[b]{0.5\textwidth}
  \[\arraycolsep=3pt\begin{array}{rlcl}
    \text{\textcolor{gray}{tile}} & \labl & \textcolor{gray}{\in} & \lbls \\
    \text{\textcolor{gray}{sort}} & \sort & \textcolor{gray}{\in} & \sorts\supseteq\{\sort^\#\}  \\
    \text{\textcolor{gray}{symbol}} & \sym & \textcolor{gray}{::=} & \labl ~\gvert~ \sort \\
    % \rzero ~\gvert~
    \text{\textcolor{gray}{regex}} & \rgx & \textcolor{gray}{::=} & \rone ~\gvert~ \sym  ~\gvert~ \ralttight{\rgx}{\rgx} ~\gvert~ \rseq{\rgx}{\rgx} ~\gvert~ \rstar{\rgx} \\
    \text{\textcolor{gray}{precedence}} & \precp,\precq & \textcolor{gray}{\in} & \precs\supseteq\{\bot,\precz,\top\} \\
    \text{\textcolor{gray}{PBG}} & \gram & \textcolor{gray}{\in} & \sorts \rightarrow \precs \rightarrow \rgx
    \vspace{-0.25cm}
  \end{array}\]
  \caption{Syntax of precedence-bounded grammars}\label{fig:pbg}
  \end{minipage}%
  \begin{minipage}[b]{0.45\textwidth}
    \[\arraycolsep=3pt\begin{array}{rlcl}
      \text{\textcolor{gray}{grout}} & \groot & \textcolor{gray}{::=} & \ophole^\sort ~\gvert~ \prehole^\sort ~\gvert~ \poshole^\sort ~\gvert~ \binhole^\sort \\
      \text{\textcolor{gray}{terminal}} & \cft & \textcolor{gray}{::=} & \droot~\gvert~ \labl ~\gvert~ \groot \\
      \text{\textcolor{gray}{nonterminal}} & \cfs & \textcolor{gray}{::=} & \scroot ~\gvert~\bddsort{\precp}{\sort}{\precq} \\
      \text{\textcolor{gray}{symbol}} & \cfx & \textcolor{gray}{::=} & \cft ~\gvert~ \cfs \\
      % \rzero ~\gvert~
      \text{\textcolor{gray}{CFG}} & \cfg,\groutgram & \textcolor{gray}{\in} & \{\cfs\mapsto\overline{\cfx}\}
      \vspace{-0.25cm}
    \end{array}\]
    \caption{Syntax of context-free grammars. \note{TODO: distinct symbols for root delimiters.}}\label{fig:cfg}
  \end{minipage}
  % \vspace{-0.25cm}
  % \caption{The syntax of \subref{fig:pbg} precedence-bounded grammars and \subref{fig:cfg} context-free grammars.}
  \vspace{0.2cm}

  \begin{minipage}[c]{0.9\textwidth}
    \centering
    \begin{minipage}[c]{0.45\textwidth}
      \vskip 0pt
      \[\arraycolsep=3pt\begin{array}{rclrl}
        \expsort & \mapsto & 1 & \mapsto & \spretile{let} ~ \patsort ~\ \sbintile{=} ~\expsort~\ \sbintile{in} ~\expsort \\
        & & 2^L & \mapsto & \expsort~\ \sbintile{+} ~\expsort ~\bvert~ \expsort~\ \sbintile{-} ~\expsort \\
        & & 3^L & \mapsto & \expsort~\ \sbintile{*} ~\expsort ~\bvert~ \expsort~\ \sbintile{/} ~\expsort \\
        & & 4 & \mapsto & \vartile{num} ~\bvert~ \vartile{var} \\
        & & & \bvert & \spretile{(} ~\expsort~(~ \sbintile{,} \expsort~)^* ~ \sposttile{)}
        \vspace{-0.2cm}
      \end{array}\]
    \end{minipage}%
    \hfill%
    \begin{minipage}[c]{0.45\textwidth}
      \vskip 0pt
      \[\arraycolsep=3pt\begin{array}{rclrl}
        \patsort & \mapsto & 1 & \mapsto & \patsort~\sbintile[\patcolor]{:}~\typsort \\
        & & 2 & \mapsto & \vartile[\patcolor]{var} \\
        & & & \bvert & \spretile[\patcolor]{(} ~\patsort~(~ \sbintile[\patcolor]{,} \patsort~)^*~ \sposttile[\patcolor]{)} \\
        \typsort & \mapsto & 1 & \mapsto & \soptile[\typcolor]{Num} \\
        & & & \bvert & \spretile[\typcolor]{(} ~\typsort~(~ \sbintile[\typcolor]{,} \typsort~)^*~ \sposttile[\typcolor]{)}
        \vspace{-0.2cm}
      \end{array}\]
    \end{minipage}%
    \subcaption{A PBG $\ghazel$ with tiles distinguished by text, shape, and color; sorts consisting of expressions, patterns, and types; and precedences consisting of associativity-tagged natural numbers}\label{fig:pbg-example}
  \end{minipage}
  % \begin{minipage}[t]{0.25\textwidth}
  %   \[\arraycolsep=3pt\begin{array}{rclrl}
  %     \vspace{-0.2cm}
  %   \end{array}\]
  % \end{minipage}
  \vspace{0.25cm}

  \begin{minipage}[c]{\textwidth}
    \centering
    \begin{tabular}{l|l|l}
      $\bddsort{\bot}{\expsort}{\bot}$ & $\bddsort{\bot}{\expsort}{3}$ & $\bddsort{3}{\expsort}{\bot}$  \\
      \cline{1-3}
      $\spretile{let}\bddsort{\bot}{P}{\bot}~\sbintile{=}\bddsort{\bot}{\expsort}{\bot}~\sbintile{in}\bddsort{1}{\expsort}{\bot}$
      &
      & $\spretile{let}\bddsort{\bot}{P}{\bot}~\sbintile{=}\bddsort{\bot}{\expsort}{\bot}~\sbintile{in}\bddsort{1}{\expsort}{\bot}$\\
      $\bddsort{\bot}{\expsort}{2}~\sbintile{+}\bddsort{2}{\expsort}{\bot}$ \hfill$\bddsort{\bot}{\expsort}{2}~\sbintile{-}\bddsort{2}{\expsort}{\bot}$
      &
      & \\
      $\bddsort{\bot}{\expsort}{3}~\sbintile{*}\bddsort{3}{\expsort}{\bot}$ \hfill $\bddsort{\bot}{\expsort}{3}~\sbintile{/}\bddsort{3}{\expsort}{\bot}$
      &$\bddsort{\bot}{\expsort}{3}~\sbintile{*}\bddsort{3}{\expsort}{\bot}$ \hfill $\bddsort{\bot}{\expsort}{3}~\sbintile{/}\bddsort{3}{\expsort}{\bot}$ &\\
      $\vartile{var}$~~$\vartile{num}$ & $\vartile{var}$~~$\vartile{num}$ & $\vartile{var}$~~$\vartile{num}$ \\
    $\spretile{(}\bddsort{\bot}{\expsort}{\bot}\sposttile{)}$\hfill $\spretile{(}\bddsort{\bot}{\expsort}{\bot}\sbintile{,}\bddsort{\bot}{\expsort}{\bot}\sposttile{)}$ $\cdots$ &
    $\spretile{(}\bddsort{\bot}{\expsort}{\bot}\sposttile{)}$\hfill $\spretile{(}\bddsort{\bot}{\expsort}{\bot}\sbintile{,}\bddsort{\bot}{\expsort}{\bot}\sposttile{)}$ $\cdots$ &
    $\spretile{(}\bddsort{\bot}{\expsort}{\bot}\sposttile{)}$\hfill $\spretile{(}\bddsort{\bot}{\expsort}{\bot}\sbintile{,}\bddsort{\bot}{\expsort}{\bot}\sposttile{)}$ $\cdots$\\
    \hline
    $\ophole^\expsort$ \hfill $\bddsort{0}{\expsort}{0}~\binhole~\bddsort{0}{\expsort}{0}$\hfill $\cdots$ & $\ophole^\expsort$ & $\ophole^\expsort$
    \end{tabular}
    \subcaption{An excerpt of the CFG $\hhazel$ compiled from the PBG in \subref{fig:pbg-example} via the rules in \autoref{fig:compile-precedence}}
    \label{fig:cfg-example}
  \end{minipage}
  \caption{\tylrcore running example: an excerpt of Hazel featuring numbers, variables, and products}
  \label{fig:gram-example}
\end{figure}


==> fig/nullable.tex <==
\begin{figure}
  \judgbox{\rnullable{\rgx}}{$\rgx$ is nullable}
  \begin{mathpar}
    \inferrule[]{
    }{
      \rnullable{\rone}
    }

    \inferrule[]{
      \rnullable{\rgx_\ell}
    }{
      \rnullable{\ralt{\rgx_\ell}{\rgx_r}}
    }

    \inferrule[]{
      \rnullable{\rgx_r}
    }{
      \rnullable{\ralt{\rgx_\ell}{\rgx_r}}
    }

    \inferrule[]{
      \rnullable{\rgx_\ell} \\
      \rnullable{\rgx_r}
    }{
      \rnullable{\rseq{\rgx_\ell}{\rgx_r}}
    }

    \inferrule[]{
    }{
      \rnullable{\rstar{\rgx}}
    }
  \end{mathpar}
  \vspace{0.2cm}

  \judgbox{\rctxnullL{\delimit}{\rctx}}{$\rctx$ has nullability $\delimit$ on its left}
  \begin{mathpar}
    \inferrule[]{
    }{
      \rctxnullL{\open}{\rctxNil}
    }

    \inferrule[]{
      \rctxnullL{\delimit}{\rctx}
    }{
      \rctxnullL{\delimit}{\rctxCons{\raltl{\rgx}}{\rctx}}
    }

    \inferrule[]{
      \rctxnullL{\delimit}{\rctx}
    }{
      \rctxnullL{\delimit}{\rctxCons{\raltr{\rgx}}{\rctx}}
    } \\

    \inferrule[]{
      \rctxnullL{\delimit}{\rctx}
    }{
      \rctxnullL{\delimit}{\rctxCons{\rseql{\rgx}}{\rctx}}
    }

    \inferrule[]{
      \rnullable{\rgx} \\
      \rctxnullL{\delimit}{\rctx}
    }{
      \rctxnullL{\delimit}{\rctxCons{\rseqr{\rgx}}{\rctx}}
    }

    \inferrule[]{
      \neg(\rnullable{\rgx})
    }{
      \rctxnullL{\closed}{\rctxCons{\rseqr{\rgx}}{\rctx}}
    }

    \inferrule[]{
      \rctxnullL{\delimit}{\rctx}
    }{
      \rctxnullL{\delimit}{\rctxCons{\rstarr}{\rctx}}
    }
  \end{mathpar}
  \caption{}
  \label{fig:nullable}
\end{figure}


==> fig/prec-rel.tex <==
\begin{figure}
  \begin{minipage}[t]{0.5\textwidth}
  \judgbox{\cmprel{\cft_\ell}{\cfs?}{\cft_r}}{}
  \begin{mathpar}
    \inferrule[]{
      \cfs\mapsto\overline{\cfx}_{\ell}\cft_{\ell}\cfs?\cft_r\overline{\cfx}_r ~\in~ \groutgram
    }{\eqrel{\cft_\ell}{\cfs?}{\cft_r}} \\

    \inferrule[]{
      \cfs\mapsto\overline{\cfx}_{\ell}\cft_{\ell}\cfs_r\overline{\cfx}_r ~\in~ \groutgram \\
      \lmt{\cfs_r}{\cfs?}{\cft_r}
    }{\ltrel{\cft_\ell}{\cfs?}{\cft_r}} \\

    \inferrule[]{
      \cfs\mapsto\overline{\cfx}_{\ell}\cfs_{\ell}\cft_r\overline{\cfx}_r ~\in~ \groutgram \\
      \rmt{\cft_\ell}{\cfs?}{\cfs_\ell}
    }{\gtrel{\cft_\ell}{\cfs?}{\cft_r}}
  \end{mathpar}
  \end{minipage}%
  \hfill%
  \begin{minipage}[t]{0.45\textwidth}%
  \judgbox{\lmt{\cfs}{\cfs?}{\cft}}{$\cft$ is a leftmost terminal of $\cfs$}
  \begin{mathpar}
    \inferrule[]{
      \derivePlus{\cfs}{\cfs?\cft\overline{\cfx}}
    }{\lmt{\cfs}{\cfs?}{\cft}}
  \end{mathpar}
  \vspace{0.45cm}

  \judgbox{\rmt{\cft}{\cfs?}{\cfs}}{$\cft$ is a rightmost terminal of $\cfs$}
  \begin{mathpar}
    \inferrule[]{
      \derivePlus{\cfs}{\overline{\cfx}\cft\cfs?}
    }{\rmt{\cft}{\cfs?}{\cfs}}
  \end{mathpar}
  \end{minipage}
  % \judgbox{\eqrel{\cft_\ell}{\cfs?}{\cft_r}}{$\cft_\ell$ has equal precedence (over $\cfs?$) to $\cft_r$}
  % \begin{mathpar}
  %   \inferrule[]{
  %     \cfs\mapsto\overline{\cfx}_{\ell}\cft_{\ell}\cfs?\cft_r\overline{\cfx}_r ~\in~ \groutgram
  %   }{\eqrel{\cft_\ell}{\cfs?}{\cft_r}}
  % \end{mathpar}

  % \judgbox{\ltrel{\cft_\ell}{\cfs?}{\cft_r}}{$\cft_\ell$ yields precedence (over $\cfs?$) to $\cft_r$}
  % \begin{mathpar}
  %   \inferrule[]{
  %     \cfs\mapsto\overline{\cfx}_{\ell}\cft_{\ell}\cfs_r\overline{\cfx}_r ~\in~ \groutgram \\
  %     \lmt{\cfs_r}{\cfs?}{\cft_r}
  %   }{\ltrel{\cft_\ell}{\cfs?}{\cft_r}}
  % \end{mathpar}

  % \judgbox{\gtrel{\cft_\ell}{\cfs?}{\cft_r}}{$\cft_\ell$ takes precedence (over $\cfs?$) over $\cft_r$}
  % \begin{mathpar}
  %   \inferrule[]{
  %     \cfs\mapsto\overline{\cfx}_{\ell}\cfs_{\ell}\cft_r\overline{\cfx}_r ~\in~ \groutgram \\
  %     \rmt{\cft_\ell}{\cfs?}{\cfs_\ell}
  %   }{\gtrel{\cft_\ell}{\cfs?}{\cft_r}}
  % \end{mathpar}
\caption{Precedence relations.}
\label{fig:prec-rel}
\end{figure}


% \begin{figure}
%   \judgbox{\eqbrel{\molbl}{\mosort?}{\molbl}}{}
%   \begin{mathpar}
%     \inferrule[]{
%       \mexit{\molbl_\ell}{\molbl_r}
%     }{
%       \eqbrel{\molbl_\ell}{\onone}{\molbl_r}
%     }

%     \inferrule[]{
%       \mexit{\mexit{\molbl_\ell}{\mosort}}{\molbl_r}
%     }{
%       \eqbrel{\molbl_\ell}{\osome{\mosort}}{\molbl_r}
%     }
%   \end{mathpar}

%   \judgbox{\ltbrel{\molbl}{\mosort}{\mosort?}{\molbl}}{}
%   \begin{mathpar}
%     \inferrule[]{
%       \menterlPlus{
%         \mexit{\molbl_\ell}{\mosort}
%         % \mosort
%       }{
%         \molbl_r
%       }
%     }{
%       \ltbrel{\molbl_\ell}{\mosort}{\onone}{\molbl_r}
%     }

%     \inferrule[]{
%       \menterlPlus{
%         \mexit{\molbl_\ell}{\mosort_\ell}
%         % \mosort_{\mathsf{up}}
%       }{
%         \mexit{\mosort_r}{\molbl_r}
%       }
%     }{
%       \ltbrel{\molbl_\ell}{\mosort_\ell}{\osome{\mosort_r}}{\molbl_r}
%     }

%     % \inferrule[]{
%     %   \mexit{\molbl_\ell}{
%     %   \ltbrel{\mosort}{}{\mosort?}{\molbl_r}
%     %   }
%     % }{
%     %   \ltbrel{\molbl_\ell}{}{\mosort?}{\molbl_r}
%     % }
%   \end{mathpar}
%   \caption{}
%   \label{fig:molded-prec-rel}
% \end{figure}


==> fig/structure.tex <==
\begin{figure}
  \begin{minipage}[t]{0.3\textwidth}
    \[\arraycolsep=3pt\begin{array}{rlrl}
      % & \chain[A, B] & \textcolor{gray}{::=} & A ~\gvert~ \chain[A, B]~B~A ~\textcolor{gray}{~\cong~}~ A~B~\chain[A, B] ~\gvert~ A \\
      \text{\textcolor{gray}{token}} & \token & \textcolor{gray}{::=} & \tnode{\cft} \\
      \text{\textcolor{gray}{term}} & \term & \textcolor{gray}{::=} & \nnode{\cfs}{\overline{\nod}} \\
      \text{\textcolor{gray}{node}} & \nod & \textcolor{gray}{::=} & \token ~\gvert~ \term \\
      \\
      \multicolumn{2}{l}{\getsym{\tnode{\cft}}} & = & \cft \\
      \multicolumn{2}{l}{\getsym{\nnode{\cfs}{\overline{\nod}}}} & = & \cfs
    \end{array}\]
    \subcaption{The syntax of terms}\label{fig:terms-syntax}
  \end{minipage}%
  \begin{minipage}[t]{0.5\textwidth}
  \centering
  \[\arraycolsep=3pt\begin{array}{rlrl}
    % & \chain[A, B] & \textcolor{gray}{::=} & A ~\gvert~ \chain[A, B]~B~A ~\textcolor{gray}{~\cong~}~ A~B~\chain[A, B] ~\gvert~ A \\
    % \text{\textcolor{gray}{token}} & \token & \textcolor{gray}{::=} & \tnode{\cft} \\
    % \text{\textcolor{gray}{term}} & \term & \textcolor{gray}{::=} & \nnode{\cfs}{\overline{\nod}} \\
    % \text{\textcolor{gray}{node}} & \nod & \textcolor{gray}{::=} & \mlbl ~\gvert~ \msort \\[0.5ex]
    \text{\textcolor{gray}{comparison}} & \cmpr & \textcolor{gray}{::=} & \lessdot ~\gvert~ \doteq ~\gvert~ \gtrdot \\[0.5ex]
    \text{\textcolor{gray}{leq}} & \cmprleq & \textcolor{gray}{::=} & \lessdot ~\gvert~ \doteq\ \ \textcolor{gray}{<:}\ \ \cmpr \\[0.5ex]
    \text{\textcolor{gray}{stack}} & \stack & \textcolor{gray}{::=} & \token ~\ \gvert~\  \stack~\cmprleq_{\term?}\token \\
    \\
    \multicolumn{2}{l}{\head{\token}} & = & \token \\
    \multicolumn{2}{l}{\head{\stack~\cmprleq_{\term?}\token}} & = & \token
\end{array}\]
  \subcaption{The syntax of stacks}
  \label{fig:stack-syntax}
  \end{minipage}%

  \begin{minipage}[t]{0.56\textwidth}
    \judgbox{\wf{\nod}}{}
    \begin{mathpar}
      \inferrule[]{
      }{
        \wf{\tnode{\cft}}
      } \\

      \inferrule[]{
        \iseq{\wf{\nod_i}}{1\leq i\leq k} \\
        \cfs\pruduce\iseq{\getsym{\nod_i}}{1\leq i\leq k}\in\groutgram
      }{
        \wf{\nnode{\cfs}{\iseq{\nod_i}{1\leq i\leq k}}}
      }
    \end{mathpar}
    \subcaption{Term well-formedness}\label{fig:terms-wf}
  \end{minipage}%
  \hfill%
  \begin{minipage}[t]{0.36\textwidth}
  \judgbox{\wf{\stack}}{}
  \begin{mathpar}
    \inferrule[]{
    }{
      \wf{\tnode{\cft}}
    } \\

    \inferrule[]{
      \wf{\stack}\\
      (\wf{\term?}\lor\term?=\none)\\
      \getsym{\head{\stack}}~\cmpr_{\getsym{\term?}}\cft
    }{
      \wf{\stack~\cmpr_{\term?}\tnode{\cft}}
    }
  \end{mathpar}
  \subcaption{Stack well-formedness}
  \label{fig:stack-wf}
  \end{minipage}%
  \caption{The syntax of terms \subref{fig:terms-syntax} and stacks \subref{fig:stack-syntax} their conditions for well-formedness, \subref{fig:terms-wf} and \subref{fig:stack-wf} respectively.}
  \label{fig:terms}

\end{figure}


==> tylrcore/grammar.tex <==
% \input{fig/grammars}

% \input{fig/grammars2}


% \begin{lemma} \label{lemma:prec-weakening}
%   If $\cfgrule{\psq}{\s{\cfx}}{\cfg}$
%   and $\precp'  \preccurlyeq_\sort \precp$ and $\precq \succcurlyeq_\sort \precq'$,
%   then $\cfgrule{\bddsort{\precp'}{\sort}{\precq'}}{\s{\cfx}}{\cfg}$.
% \end{lemma}


% \subsubsection{Adding Grout Rules} \label{sec:adding-grout}



% \subsubsection{Precedence Chains}




% A nonterminal $\cfsr$ is called \emph{$\sort$-groutable}
% for some sort $\sort$ if $\zerosort{\sort} \yieldsop^* \cfsr$.
% A term $\termr$ is called \emph{$\sort$-groutable}
% if $\termr\Reduce\cfsr$ and $\cfsr$ is $\sort$-groutable.
% Nonterminals and terms are called \emph{groutable} if they are $\startSym$-groutable.

% \begin{lemma}
% Bounded sort $\psq$ is $\startSym$-groutable
% if and only if
% $\glp\sort\neq\startSym$
% or $\glp\precz \preccurlyeq_{\startSym} \precp$
% and $\precq \succcurlyeq_{\startSym} \precz\glr\glr$.
% \end{lemma}

% \begin{lemma}
% For all right-concave grout $\groot$
% and $\startSym$-groutable nonterminals $\cfsr$,
% there exists $\cfs$ such that
% $\groot^{\startSym} \adjop \cfs \bounds \cfsr$.
% \end{lemma}

% \begin{lemma} \label{lemma:root-grout-prec'}
%   If grout $\groot$ is right-concave,
%   then for any $\startSym$-groutable slot $\cfsr?$
%   and tile $\labl$,
%   there exist slots $\iseq{\o{\cfs}_i}{0\leq i \leq k}$
%   and terminals $\iseq{\cft_i}{0\leq i \leq k}$
%   such that
%   $\groot^{\startSym}
%   \iseq{\cmprleq_{\o{\cfs}_i}\cft_i}{0\leq i \leq k}
%   = \labl$
%   and $\o{\cfsr} = \o{\cfs}_j$
%   for some $0\leq j \leq k$.
% \end{lemma}



% \begin{lemma}[Lonely $\scroot$] \label{lemma:lonely-scroot}
%   There exists no symbol $\cfx$ such that $\scroot \adjop \cfx$ or $\cfx \adjop \scroot$.
% \end{lemma}

% \begin{lemma}[Nonterminals are Zero-Reachable]
% \label{lemma:nonterminals-zero-reachable}
%   For all bounded sorts $\cfs = \psq$,
%   if $\sort \neq \startSym$
%   or \glp$\precz \preccurlyeq_{\startSym} \precp$
%   and $\precq \succcurlyeq_{\startSym} \precz$\glr,
%   then $\yieldsStar{\zerosort{\startSym}}{\cfs}$.
% \end{lemma}

% \begin{lemma} \label{lemma:cltop-dlroot}
% If $\cfs ~\cltop{\o{\cfs}}~ \dlroot$, then $\cfs = \scroot$ and $\o{\cfs} = \none$.
% \end{lemma}
% \begin{lemma} \label{lemma:drroot-cgtop}
% If $\drroot ~\cgtop{\o{\cfs}}~ \cfs$, then $\cfs = \scroot$ and $\o{\cfs} = \none$.
% \end{lemma}
% \begin{lemma} \label{lemma:no-trespassing}
% There exists no $\cft$ and $\cmpr$ such that $\cft\cmpr\dlroot$ or $\drroot\cmpr\cft$.
% \end{lemma}
% \begin{lemma} \label{lemma:no-escaping}
% There exists no $\cft$ such that $\cft \lessdot \drroot$ or $\dlroot \gtrdot \cft$.
% \end{lemma}

% \subsubsection{Bounds}


% \begin{lemma} \label{lemma:lt-bot-witness'}
%   If $\cft \adjop \psq \lmsymop^* \cfs$
%   then $\cft \adjop \bddsort{\precp}{\sort}{\bot} \lmsymop^* \cfs$.
% \end{lemma}

% \begin{proof}
%   Apply Lemma \ref{lemma:adj-bot}
%   to $\cft \adjop \psq$
%   to get $\adj{\cft}{\bddsort{\precp}{\sort}{\bot}}$.
%   Since $\precq \pgeq_\sort \bot$, use \texttt{PElab-Weaken}
%   to turn $\psq \lmsymop^* \cfs$
%   into $\bddsort{\precp}{\sort}{\bot} \lmsymop^* \cfs$.
% \end{proof}


% \begin{lemma}
% If $\psq \produce \s{\cfx}$
% there exists a unique maximal pair of bounds $\precp_0, \precq_0$
% such that $\precp \preccurlyeq_\sort \precp_0$
% and $\precq_0 \succcurlyeq_\sort \precq$
% and $\bddsort{\precp_0}{\sort}{\precq_0} \produce \s{\cfx}$.
% \end{lemma}

% \begin{lemma} \label{lemma:bounded-sort-tile}
%   If $\cfs \produce \dots\labl\dots$ then $\cfs =
%   \psq$ for some sort
%   $\sort$ and precedence bounds $\precp, \precq$.
% \end{lemma}

% \begin{lemma} \label{lemma:bounded-sort-grout}
%   If $\cfs \produce \dots\groot^\sort\dots$ then $\cfs =
%   \psq$ for some precedence bounds $\precp, \precq$.
% \end{lemma}

% \begin{lemma} \label{lemma:construct-snug}
%   If $\s{\nod} = {\nod_L\dots} = {\dots\nod_R}$
%   and $\nod_L$ is snug on the left
%   and $\nod_R$ is snug on the right
% \end{lemma}

\newcommand{\pwls}[1]{\mathrel{\prescript{}{#1}{\!\pwl}}}%
\newcommand{\pwrs}[1]{\pwr_{#1}}%
% \begin{figure}[h]
%   \centering
%   % \judgbox{\pwl \term}{$\term$ is snug on the left}
%   % \begin{mathpar}
%   %   \inferrule{
%   %     \getsym{\nod} \neq \bddsort{\medsquare}{\sort}{\medsquare}
%   %   }{\pwl \nnode{\bddsort{\top}{\sort}{\precq}}{\nod\dots}}

%   %   \inferrule{
%   %     \pwl \term \\
%   %     \getsym{\term} = \bddsort{\medsquare}{\sort}{\medsquare}
%   %   }{
%   %     \pwl
%   %     \nnode{\bddsort{\bot}{\sort}{\medsquare}}
%   %     {\term\groot^\sort\dots}
%   %   }

%   %   \inferrule{
%   %     \pwl \term \\
%   %     \getsym{\term} = \bddsort{\medsquare}{\sort}{\medsquare} \\
%   %     {\sort\labl\dots} \in \rgxsem{\gram(\sort,\precp)}
%   %   }{
%   %     \pwl
%   %     \nnode{\bddsort{\precp}{\sort}{\medsquare}}
%   %     {\term\labl\dots}
%   %   }
%   % \end{mathpar}%
%   \judgbox{\s\nod \pwrs{\sort} \precq}{Nodes $\s\nod$ synthesize bound $\precq$ of sort $\sort$ on the right}%
%   \begin{mathpar}
%     \inferrule{
%       % {\dots\labl\dots} \in \rgxsem{\gram(\sort,\medsquare)}
%     }{\dots\token \pwrs{\sort} \top}

%     \inferrule{
%       \sortr \neq \sort
%     }{\dots\nnode{\bddsort{\medsquare}{\sortr}{\medsquare}}{\medsquare} \pwrs{\sort} \top}

%     % \inferrule{
%     %   % \term \pwrs{\sort} \precq
%     % }{\nnode{\bddsort{\medsquare}{\sort}{\medsquare}}{\dots\token} \pwrs{\sort} \top}

%     \inferrule{
%       % \term \pwrs{\sort} \precq
%     }{\dots\groot^{\sort}\term \pwrs{\sort} \bot}

%     \inferrule{
%       {\dots\labl\sort} \in \rgxsem{\gram(\sort,\precp)} \\
%       \s\nod \pwrs{\sort} \precq
%     }{\dots\labl\nnode{\bddsort{\medsquare}{\sort}{\medsquare}}{\s\nod} \pwrs{\sort} \min(\precp,\precq)}
%   \end{mathpar}%
%   % \judgbox{\precp \pwl \sort \deriveop \s\nod}{
%   %   $\precp$ snugly bounds nodes $\s\nod$ of sort $\sort$ on the left}
%   % \begin{mathpar}
%   %   \inferrule{
%   %   }{\top \pwl \sort \deriveop \token\dots}

%   %   \inferrule{
%   %     \sort \neq \sortr
%   %   }{\top \pwl \sort \deriveop \nnode{\bddsort{\medsquare}{\sortr}{\medsquare}}
%   %   {\medsquare}\dots} \\

%   %   \inferrule{
%   %     \sort \neq \sortr
%   %   }{\top \pwl \sort \deriveop \nnode{\bddsort{\medsquare}{\sortr}{\medsquare}}
%   %   {\medsquare}\dots}

%   %   \inferrule{
%   %     \getsym{\nod} \neq \bddsort{\medsquare}{\sort}{\medsquare}
%   %   }{\top \pwl \sort \deriveop \nod\dots}

%   %   \inferrule{
%   %     \pwl \term \\
%   %     \getsym{\term} = \bddsort{\medsquare}{\sort}{\medsquare}
%   %   }{
%   %     \pwl
%   %     \nnode{\bddsort{\bot}{\sort}{\medsquare}}
%   %     {\term\groot^\sort\dots}
%   %   }

%   %   \inferrule{
%   %     \preco \pwl \sort \deriveop \s\nod
%   %   }{
%   %     \min(\preco,\precq)
%   %     \pwl \sort \deriveop
%   %     \nnode{\bddsort{\precp}{\sort}{\pincl{\sort}\precq}}{\s\nod}\dots
%   %   }
%   % \end{mathpar}
%   % \judgbox{\sort \deriveop \s\nod \pwr \precq}{
%   %   $\precq$ tightly bounds nodes $\s\nod$ of sort $\sort$ on the right}
%   % \begin{mathpar}
%   %   \inferrule{
%   %     \getsym{\nod} \neq \bddsort{\medsquare}{\sort}{\medsquare}
%   %   }{\sort \deriveop \dots\nod \pwr \top}

%   %   \inferrule{
%   %     \sort \deriveop \s\nod \pwr \preco
%   %   }{
%   %     \sort \deriveop \dots\nnode{\bddsort{\precp\pincr{\sort}}{\sort}{\precq}}{\s\nod} \pwr \min(\precp,\preco)
%   %   }
%   % \end{mathpar}
% \end{figure}

% \begin{definition}
% A term $\term = \nnode{\psq}{\s{\nod}}$ is called \emph{snug}
% if $\precp \pwls{\sort} \s\nod \pwrs{\sort} \precq$.
% \end{definition}


% \begin{lemma} \label{lemma:unique-disputes-star}
%   If $\psq \lmsymop^* \bddsort{\medsquare}{\sort}{\preco_1}$
%   and $\psq \lmsymop^* \bddsort{\medsquare}{\sort}{\preco_2}$
%   then $\preco_1 = \preco_2$.
% \end{lemma}

% There exist no regexes $\rgx_L = \gram(\sort_L, \precp_L)$ and $\rgx_R = \gram(\sort_R, \precp_R)$
% such that $\sort_L \neq \sort_R$
% and ${\sort_L\dots}\in\rgxsem{\rgx_R}$
% and ${\dots\sort_R}\in\rgxsem{\rgx_L}$.
% There exist no sorts $\sort_L, \sort_R\in\sorts$ and precedence levels $\precp_L, \precp_R\in\precs$ such that $\sort_L \neq \sort_R$ and ${\sort_R\dots}\in\rgxsem{\gram(\sort_L, \precp_L)}$ and ${\dots\sort_L}\in\rgxsem{\gram(\sort_R, \precp_R)}$.



==> tylrcore/parsing.tex <==
\subsection{Parsing} \label{sec:tylrcore-parsing}




% \begin{lemma}
%   For any tile $\labl$, there exist terminals $\iseq{\cft_i}{1\leq i\leq k}$ and cells $\iseq{\o{\cfs}_i}{1\leq i\leq k}$  ($k\geq 1$) such that $\cft_k = \labl$ and $\dlroot \iseq{\cmprleq_{\o{\cfs}_i} \cft_i}{1\leq i\leq k}$.
% \end{lemma}

% \begin{lemma}
% If $\yieldsPlus{\cfs}{\cft}$ then there exists $\cft_L$ such that $\lmt{\cfs}{}{\cft_L} ~\ceqop{}^*~ \cft$.
% \end{lemma}

% \begin{lemma} \label{lemma:droot-top}
% There exists no $\cfs$ such that $\cfs \cltop{} \drroot$ or $\dlroot \cgtop{} \cfs$.
% \end{lemma}

% \begin{lemma}[Coherence]
% \label{lemma:coherence}
% If $\cfs ~\clessdot_{\o{\cfs}_0} \cft_0 \iseq{\ceqop{\o{\cfs}_i} \cft_i}{1\leq i\leq n}~\cgtrdot_{\o{\cfs}_{n+1}} \cfs$, then $\derive{\cfs}{\iseq{{\o{\cfs}_i} \cft_i}{0\leq i\leq n}\o{\cfs}_{n+1}}$.
% \end{lemma}

% \begin{proof}
% The premises
% \begin{align}
%   \cfs ~\clessdot_{\o{\cfs}_0} \cft_0\ , \label{eq:clt0}\\
%   \iseq{\cft_i \ceqop{\o{\cfs}_i} \cft_{i+1}}{0\leq i\leq n}\ , \\
%   \cft_{n+1} ~\cgtrdot_{\o{\cfs}_{n+1}} \cfs\
% \end{align}
% imply there exist nonterminals $\cfs = \psq$ and
% $\iseq{\cfs_i = \bddsort{\precp_i}{\sort_i}{\precq_i}}{0\leq i\leq n}$ such that
% \begin{align}
%   % \cfgrule{\psq}{\o{\cfs}_0 \cft_0 \dots}{\groutgram} \label{eq:lt0} \\
%   % \iseq{
%   %   \cfgrule{\bddsort{\precp_i}{\sort_i}{\precq_i}}{\dots \cft_i \o{\cfs}_i \cft_{i+1}  \dots}{\groutgram}
%   % }{0\leq i \leq n} \\
%   % \cfgrule{\psq}{\dots \cft_{n+1}\o{\cfs}_{n+1}}{\groutgram}
%   \deriveStar{\cfs}{\o{\cfs}_0 \cft_0 \dots} \label{eq:lt0} \\
%   \iseq{
%     \cfgrule{\cfs_i}{\dots \cft_i \o{\cfs}_i \cft_{i+1}\dots}{\groutgram}
%   }{0\leq i < n} \label{eq:eqi}\\
%   \deriveStar{\cfs}{\dots \cft_{n}\o{\cfs}_{n+1}}
% \end{align}
% Proceed by case analysis on $\cft_0$. We know by Lemma \ref{lemma:droot-top} applied to \eqref{eq:clt0} that $\cft_0 \neq \drroot$.
% \begin{itemize}
% \item Suppose $\cft_0 = \dlroot$. Combining Lemmas \ref{lemma:droot-eq}, \ref{lemma:cltop-dlroot}, \ref{lemma:drroot-cgtop}, and \ref{lemma:droot-top}, we have that $n = 1$, $\cfs = \scroot$, $\o{\cfs}_0 = \none$, $\cft_0 = \dlroot$, $\o{\cfs}_1 = \botsort{\startSym}$, $\cft_1 = \drroot$, and $\o{\cfs}_{2} = \none$.
% Rules \texttt{PElab-Root} and \texttt{GInj-Include} give us $\derive{\scroot}{\dlroot~\botsort{\startSym}~\drroot}$.
% \item Suppose $\cft_0 = \groot_0^{\sort'}$.
% By Lemma \ref{lemma:homogeneity} applied to \eqref{eq:eqi}, we have that $\cft_i = \groot_i^{\sort'}$ for all $0\leq i\leq n$.
% \note{todo: existing proof assumed closed ops were single-step yields}
% \end{itemize}
% \end{proof}

% \begin{lemma}[Fill Preserves Well-Formedness]
% \label{lemma:fill-wf}
% If $\wf{\o{\term}}$ and $\pfill{\o{\term}}{\o{\cfs}}=\o{\termr}$, then
% $\wf{\o{\termr}}$.
% \end{lemma}

% \begin{lemma}[Empty Fill]
%   \label{lemma:fill-empty}
%   For all $\s{\o{\cfs}}$, there exists $\s{\o{\term}}$ such that $\pick{\none}{\s{\o{\cfs}}}{\s{\o{\term}}}$.
% \end{lemma}

% \begin{lemma}[Fill Root] \label{lemma:root-fillable}
%   % For every bounded-sorted term $\term =
%   % \nnode{\psq}{\s{\nod}}$,
%   % there exists $\termr$
%   % such that $\pick{\term}{\botsort{\startSym}}{\termr}$.
%   For every term $\termr$,
%   there exists term $\term$
%   such that $\pick{\some{\termr}}{\some{\botsort{\startSym}}}{\some{\term}}$.
% \end{lemma}

% \begin{lemma}[Left-Bounded Fill]\label{lemma:fill-success}
%   % For all bounded sorts $\cfs = \bddsort{\preco}{\sort}{\bot}$
%   % and terms $\termr$
%   % such that $\cfs \lmsymop^* \getsym{\termr}$,
%   % there exists $\term$
%   % such that $\pick{\some{\termr}}{\some{\cfs}}{\some{\term}}$.
%   For all nonterminals $\cfs = \bddsort{\precp}{\sort}{\bot}$ and terms $\termr$
%   such that $\cfs \lmsymop^* \cfsr \Produce \termr$,
%   there exists term $\term$
%   such that $\pick{\some{\termr}}{\some{\cfs}}{\some{\term}}$.
% \end{lemma}

% \begin{proof}
% % Let $\termr = \snode{\s{\nod}}$.
% Let $\rho = \bddsort{\precm}{\sortr}{\precn}$.
% Assume the premises:
% \begin{align}
%  \cfs = \bddsort{\precp}{\sort}{\bot} \lmsymop^* \bddsort{\precm}{\sortr}{\precn} = \rho \Produce \termr \label{eq:fill-success-lmsym}
% \end{align}

% Suppose $\sortr = \sort$.
% It suffices by rule \texttt{Fill-Bounded}
% to show $\cfs \Produce \termr$.
% It suffices by \Lemmaref{lemma:loosen-produce}
% to show $\cfs \bounds \rho$,
% \ie $\precp \pleq_\sort \precm$
% and $\precn \pgeq_\sort \bot$.
% The first follows by Lemma \ref{lemma:dispute-inherit-star}
% applied to \eqref{eq:fill-success-lmsym},
% the second by definition.

% Suppose $\sortr \neq \sort$.
% It suffices by rule \texttt{Fill-Grout-R}
% to show $\cfs \Produce \snode{\termr\,\poshole^\sort}$.
% Given $\rho \Produce \termr$ in \eqref{eq:fill-success-lmsym},
% it suffices by rule \texttt{Produce-Term}
% to show that $\cfs \produce \cfsr\,\poshole^\sort$.
% It suffices by rules \texttt{Produce-Loosen} and \texttt{Produce-Subsume}
% to show $ \topsort{\sort}\reduce\cfsr\,\poshole^\sort$.
% It suffices by rule \texttt{GInj-Postfix} $\glp\textcolor{gray}{k = 0}\glr$
% to show $\lmsymStar{\zerosort{\sort}}{\cfsr}$.
% \note{todo: finish.}
% % Apply Lemma \ref{lemma:unbounded-sort-transition}
% % to \eqref{eq:fill-success-lmsym}
% % to get $\bddsort{\preco}{\sort}{\bot} \lmsymop^* \botsort{\sortr}$.
% % Apply \texttt{GInj-Postfix} $\glp\textcolor{gray}{k = 0}\glr$ to get
% % \begin{align}
% %   \syninj{\gram}{\botsort{{\sortr}}\,\poshole^{\sort}}{\topsort{\sort}}
% %   \label{eq:fill-success-cfgrule}
% % \end{align}
% % Apply \texttt{GInj-Weaken} to \eqref{eq:fill-success-cfgrule} to get
% % \begin{align}
% %   \cfgrule{
% %     \bddsort{\preco}{\sort}{\bot}
% %   }{\botsort{\sortr}\,\poshole^{\sort}}{\cfg}
% %   \label{eq:fill-success-cfgrule-weaken}
% % \end{align}
% % Apply \texttt{Fill-Grout-R} to \eqref{eq:fill-success-cfgrule-weaken}
% % to get
% % $\pick{\some{\termr}}{\some{\cfs}}{\some{\nnode{\bddsort{\preco}{\sort}{\bot}}{\nnode{\botsort{\sortr
% % }}{\s{\nod}}\,\poshole^{\sort}}}}$.
% \end{proof}

% \begin{lemma}[Root Shiftability]\label{lemma:root-shiftability}
% If $\reachable{\pushl{\droot}{\o{\term}}{\

% \subsubsection{Validity}


% \input{\chpath/validity}

% \begin{lemma} \label{lemma:tight-tiles}
% If $\pwl \nnode{\psq}{\s{\nod}} \pwr$,
% and there exists no grout $\groot$
% such that $\groot^\sort \in \s{\nod}$,
% then $0 \pleq_\sort \precp$ and $\precq \pgeq_\sort 0$.
% \end{lemma}


==> tylrcore/validity.tex <==
% \begin{lemma}[Push Validity] \label{lemma:push-wf}
%   If $\wf{\stack}$
%   and $\tilepushed{\stack}$
%   and $\pushedcft{\cft}$
%   and $\push{\stack}{\none}{\cft}{\stack'}$,
%   then $\wf{\stack'}$ and $\tilepushed{\stack'}$.
% \end{lemma}
% \begin{proof}
% Corollary of the generalization to Lemma \ref{lemma:push-wf'}.
% \end{proof}

\begin{lemma}[Reduce Preserves Well-Formedness]
\label{lemma:reduce-preserves-wf}
Let $\stack$
$\cfs \produce \iseq{\o{\cfsr}_i\,\labl_i}{0 \leq i \leq n}\,\o{\cfsr}_{n+1}$
and
$\iseq{\o{\cfsr}_i \Produce \o{\termr}_i}{0\leq i\leq k}$
$\pfill{\s{\termr}}{\iseq{\o{\cfsr}_i}{k < i \leq n+1}} = {\iseq{\o{\term}_i}{k < i \leq n+1}}$
\end{lemma}

\begin{lemma}[Push Validity] \label{lemma:push-wf}
  If $\wf{\pushl{\stack}{\s{\termr}}{\medsquare}}$
  and $\push{\stack}{\s{\termr}}{\cft}{\stack'}$
  then $\wf{\stack'}$.
\end{lemma}

\begin{proof}
Assume and invert the premise $\wf{\pushl{\stack}{\s{\termr}}{\medsquare}}$ to
get slot $\o\cfsr$ and cell $\o\termr$ such that
\begin{align}
\wf{\stack} \label{eq:wf-stack} \\
\head{\stack} \adjop \o\cfsr \label{eq:stack-adj-cfsr} \\
\pfill{\s\termr}{\o\cfsr} = \o\termr \label{eq:stack-fill}
\end{align}
Proceed by induction on $\push{\stack}{\s{\termr}}{\cft}{\stack'}$.
\begin{itemize}
  \item Case \texttt{Shift}$\;\glp\textcolor{gray}{k \geq 0}\glr$:
  \begin{align}
    \head{\stack}\iseq{\cmprleq_{\dsty{\o{\cfs}_i}}\cft_i}{0\leq i\leq k} = \cft \label{eq:shift-leq} \\
    \pfill{\s{\termr}}{\iseq{\o{\cfs}_i}{0\leq i\leq k}} = {\iseq{\o{\term}_i}{0\leq i\leq k}} \label{eq:shift-fill} \\
    \stack' \,=\, \stack\iseq{\cmprleq_{\dsty{\o{\term}_i}}\cft_i}{0\leq i\leq k}
  \end{align}
  \Lemmaref{lemma:fill-wf} applied to \eqref{eq:shift-fill} gives us
  \begin{align}
    \iseq{\o{\cfs}_i \Produce \o{\term}_i}{0\leq i\leq k} \label{eq:shift-syms}
  \end{align}
  Using \eqref{eq:shift-leq} and \eqref{eq:shift-syms},
  apply \texttt{WFStack-Cons} to \eqref{eq:wf-stack} $k+1$ times in succession to get $\wf{\stack'}$.

  % It remains to show that $\tilepushed{\stack'}$.
  % Inverting the premise $\reachable{\pushl{\medsquare}{\o{\term}}{\cft}}$ gives us
  % $\cft_k = \cft$ is not grout.
  % If some $\cft_j$ for some $1 \leq j < k$ is right-convex grout,
  % then applying Lemma \ref{lemma:grout-prec}
  % to $\cft_j \cmprleq_{\o{\cfs}_{j+1}} \cft_{j+1}$ leads to absurdity.
  % Therefore, starting with $\tilepushed{\stack}$, we can apply
  % \texttt{NoRCG-Cons} $k$ times in succession to get $\tilepushed{\stack'}$.

  \item Case \texttt{Reduce}$\;\glp\textcolor{gray}{0 \leq k \leq n}\glr$:
  \begin{align}
    \stack \,=\, \stack_0
    \lessdot_{\dsty{\o{\termr}_0}}\labl_0
    \iseq{\doteq_{\dsty{\o{\termr}_i}}\labl_i}{0\leq i\leq k} \\
    % k \leq n \\
    % \head{\stack_0} ~\adjop~ \cfs_{\stack_0} ~\lmsymop^*~ \cfs \label{eq:reduce-adj-lmsym}\\
    % \derive{\cfs}{\iseq{\getsym{\o{\term}_i}~\cft_i}{0\leq i\leq k}\iseq{\o{\cfs}_i\cft_i}{k < i \leq n}\o{\cfs}_{n+1}} \label{eq:reduce-derive} \\
    \cfs \produce \iseq{\o{\cfsr}_i\,\labl_i}{0 \leq i \leq n}\,\o{\cfsr}_{n+1}
    \label{eq:reduce-derive} \\
    \iseq{\o{\cfsr}_i \Produce \o{\termr}_i}{0\leq i\leq k} \\
    \pfill{\s{\termr}}{\iseq{\o{\cfsr}_i}{k < i \leq n+1}} = {\iseq{\o{\termr}_i}{k < i \leq n+1}} \label{eq:reduce-fill} \\
    % \term' = \snode{\o{\term}_0\iseq{\tnode{\cft_i}~\o{\term}_{i+1}}{0\leq i\leq n}} \\
    \push{\stack_0}{\displaystyle{\snode{\o{\termr}_0\iseq{\labl_i\,\o{\termr}_{i+1}}{0\leq i\leq n}}}}{\cft}{\stack'}
  \end{align}
  Let $\term = \snode{\o{\termr}_0\iseq{\tnode{\labl_i}~\o{\termr}_{i+1}}{0\leq
  i\leq n}}$.
  To show $\wf{\stack'}$,
  it suffices by our inductive hypothesis to show
  $\wf{\pushl{\stack_0}{\term}{\medsquare}}$,
  for which it suffices in turn to show
  there exists nonterminal $\cfs$ and cell $\o{\term}$ such that
  % there exists nonterminal $\cfsr$ and sort $\sortr$ such that
  \begin{align}
    \wf{\stack_0} \label{eq:stack0-wf} \\
    % \zerosort{\sortr} \bounds \cfsr \Reduce \term \label{eq:reduce-term-natural}
    \head{\stack_0} \adjop \cfs \label{eq:stack0-adj-cfs} \\
    \pfill{\term}{\some{\cfs}} = \o\term
  \end{align}
  % \eqref{eq:reduce-tilepushed} follows from $k+1$ inversions of
  % $\texttt{NoRCG-Cons}$ on the assumption $\tilepushed{\stack}$.
  Starting with \eqref{eq:wf-stack}, invert \texttt{WFStack-Cons} $k+1$ times in
  succession to get \eqref{eq:stack0-wf} and
  \begin{align}
    % \wf{\stack_0} \label{eq:reduce-wf-stack-0} \\
    \iseq{\o{\cfs}_i \Produce \o{\term}_i}{0\leq i\leq k} \label{eq:reduce-wf-term-0-k}
  \end{align}
  Apply \Lemmaref{lemma:fill-wf} to \eqref{eq:reduce-fill} to get
  \begin{align}
    \iseq{\o{\cfs}_i \Produce \o{\term}_i}{k < i \leq n+1} \label{eq:reduce-wf-term-k-n}
  \end{align}
  Apply \texttt{Produce-Term} to \eqref{eq:reduce-derive} and \eqref{eq:reduce-wf-term-0-k} and
  \eqref{eq:reduce-wf-term-k-n} to get
  \begin{align}
    \cfs \Produce \term \label{eq:cfs-produce-term}
  \end{align}
  Apply \Lemmaref{lemma:produce-iff-reduce} to \eqref{eq:cfs-produce-term}
  to get nonterminal $\cfsr$ such that $\cfsr\Reduce\term$,
  to which applying \Lemmaref{lemma:natural-terms} gives sort $\sortr$
  such that $\cfsr \bounded \zerosort{\sortr}$,
  altogether giving \eqref{eq:reduce-term-natural}.
\end{itemize}
\end{proof}

\begin{theorem}[Parsing Validity]
For any tile sequence $\iseq{\tnode{\labl_i}}{1\leq i\leq k}$, if
\[
\parse{\dlroot}{\iseq{\tnode{\labl_i}}{1\leq i\leq k}~\tnode{\drroot}}{
  \dlroot\doteq_{\term}\drroot
}
\]
then $\wf{\term}$.
\end{theorem}

